Towards Verified and Targeted Explanations through Formal Methods

As deep neural networks are deployed in safety-critical domains such as autonomous driving and medical diagnosis, stakeholders need explanations that are interpretable but also trustworthy with formal guarantees. Existing XAI methods fall short: heuristic attribution techniques (e.g., LIME, Integrated Gradients) highlight influential features but offer no mathematical guarantees about decision boundaries, while formal methods verify robustness yet remain untargeted, analyzing the nearest boundary regardless of whether it represents a critical risk. In safety-critical systems, not all misclassifications carry equal consequences; confusing a "Stop" sign for a "60 kph" sign is far more dangerous than confusing it with a "No Passing" sign. We introduce ViTaX (Verified and Targeted Explanations), a formal XAI framework that generates targeted semifactual explanations with mathematical guarantees. For a given input (class y) and a user-specified critical alternative (class t), ViTaX: (1) identifies the minimal feature subset most sensitive to the y->t transition, and (2) applies formal reachability analysis to guarantee that perturbing these features by epsilon cannot flip the classification to t. We formalize this through Targeted epsilon-Robustness, certifying whether a feature subset remains robust under perturbation toward a specific target class. ViTaX is the first method to provide formally guaranteed explanations of a model's resilience against user-identified alternatives. Evaluations on MNIST, GTSRB, EMNIST, and TaxiNet demonstrate over 30% fidelity improvement with minimal explanation cardinality.

==> diagrams/ReachX_diagram.tex <==
\begin{tikzpicture}
% heuristic search
\node[draw, fill=blue!40, rectangle, minimum width=4cm, minimum height=2cm, align=center, font=\large] at (0,0) (heuristic_search){Heuristic Search};
% theta, s
\node[right=of heuristic_search, font=\large, yshift=0.4cm, xshift=-0.75cm] {$\theta$};
\node[right=of heuristic_search, font=\large,  yshift=-0.4cm, xshift=-1.1cm] {$s=0$};
% binary search
\node[draw, fill=blue!40, rectangle, minimum width=4cm, minimum height=2cm, align=center, font=\large, right=of heuristic_search] (bin_search) {Binary* Search};
% A, B
\node[right=of bin_search, font=\large, yshift=0.7cm, xshift=-0.75cm] {A};
\node[right=of bin_search,font=\large, yshift=-0.7cm, xshift=-0.75cm] {B};


%
% inputs
%
\node[left=of heuristic_search, font=\large, yshift=-0.4cm] (f) {$f$};
\node[left=of heuristic_search, font=\large, yshift=0.4cm]  (x) {$x$};
\node[above=2.5cm of x, font=\large] (z) {$z$};
\node[above=0.25 of z, font=\large] (eps){$\epsilon$};
\node[above=0.25 of eps, font=\large] (delta){$\delta$};

%
% Perturbations
%
\node[draw, fill=blue!40, rectangle, minimum width=4cm, minimum height=2cm, align=center, font=\large, right=1cm of z, xshift=0.05cm] (perturbations) {Generate\\$\epsilon$-Perturbation};
\node[right=0.2cm of perturbations, yshift=0.3cm] {$X_{\epsilon}$};


%
% reachability
%
\node[draw, fill=blue!40, rectangle, minimum width=4cm, minimum height=2cm, align=center, font=\large, right=of bin_search] (reach) {$\mathcal{V}$};

%
% delta sensitive features
% 
\node[draw, fill=blue!40, diamond, minimum width=5cm, minimum height=2cm, align=center, font=\large, right=of reach] (delta_sensitive) {};
\node[align=center, font=\large] at ($(delta_sensitive) + (0, -0.1)$) {$\delta$-sensitive features\\or timeout?};

%
% restart bin search
%
\draw[->] (delta_sensitive) -- ($(delta_sensitive.south) + (0, -0.75)$) -- ($(delta_sensitive.south) + (-10.53, -0.75)$) -- (bin_search.south);


%
% Success means leave
%
\draw[->] (delta_sensitive) -- ($(delta_sensitive.east) + (3.0, 0)$);





% Arrows
\draw[->] (x) -- ($(heuristic_search.west) + (0, 0.4)$);
\draw[->] (f) -- ($(heuristic_search.west) + (0, -0.4)$);
\draw[->] (heuristic_search) -- (bin_search);
\draw[->] ($(bin_search.east) + (0, 0.4)$) -- ($(reach.west) + (0, 0.4) $);
\draw[->] ($(bin_search.east) + (0, -0.4)$) -- ($(reach.west) + (0, -0.4) $);
\draw[->] (z) -- (perturbations);
\draw[->] (eps) -- ($(perturbations.west) + (0, 0.66)$);
\draw[->] ($(x.east) + (0.6, 0)$) -- ($(x.east) + (0.6, 2.3)$) -- ($(perturbations.west) + (0, -0.63)$);
\draw[->] (perturbations) -- ($(reach.north) + (-1.0, 2.3)$) -- ($(reach.north) + (-1.0, 0)$) ;

\draw[->] (delta) -- ($(delta.east) + (13.05, 0)$) -- (reach.north);
\draw[->] (reach) -- (delta_sensitive);

% Helper labels

\node[font=\large] at ($(reach.north) + (0.3, 0.4)$) {$\delta$};
\node[font=\large] at ($(reach.north) + (-1.5, 0.4)$) {$X_{\epsilon}$};
\node[font=\large] at ($(delta_sensitive.west) + (-1.2, -2.2)$) (no) {no};
\node[font=\large] at ($(delta_sensitive.east) + (0.4, 0.3)$) (yes) {yes};
\node[font=\large] at ($(delta_sensitive.west) + (-1.2, -1.4)$) {$s = s + 1$};
\node[font=\large] at ($(delta_sensitive.east) + (3.0, 0.4)$) {$A$};


%
% Background
%
    % \coordinate (right_ext) at ([xshift=cm]reach.east); % Adjust xshift to control the extension
    % \coordinate (bottom_ext) at ([yshift=1.5]no.south); % Adjust xshift to control the extension
    % \coordinate (top_ext) at ([yshift=1.0]perturbations.north); % Adjust xshift to control the extension

    \node[above=0.5cm of perturbations,] (top_fill){}; 
    \node[left=0.2cm of heuristic_search] (left_fill){}; 

    % Background box with rounded corners, dashed line, and filled with transparent light blue
    \begin{scope}[on background layer]
        \node[fit=(heuristic_search) (bin_search) (perturbations) (reach) (delta_sensitive) (left_fill)(top_fill) (no)(yes), draw=blue, dashed, fill=blue!10, thick, inner sep=10pt, rounded corners] (xreach) {};
    \end{scope}

    \node[above=0.5cm of xreach, font=\Large, xshift=-8.25cm] {\textbf{ReachX Explainability}}; 
    


\end{tikzpicture}


==> results/eval_table_comprehensive.tex <==
% Please add the following required packages to your document preamble:
% \usepackage{multirow}

% \begin{figure}[!ht]
%     \centering

%     \begin{subfigure}[t]{0.09\textwidth}
%         \centering
%         \includegraphics[width=\textwidth]{diagrams/qualitative_result_for_experiment/mnist/ViTaX.png}
%         \caption*{ViTaX \newline}
%     \end{subfigure}
%     % \hfill
%     % \begin{subfigure}[t]{0.075\textwidth}
%     %     \centering
%     %     \includegraphics[width=\textwidth]{diagrams/qualitative_result_for_experiment/mnist/ViTaX_relax.png}
%     %     \caption*{ViTaX Relax50\%}
%     % \end{subfigure}
%     \hfill
%     \begin{subfigure}[t]{0.09\textwidth}
%         \centering
%         \includegraphics[width=\textwidth]{diagrams/qualitative_result_for_experiment/mnist/verix.png}
%         \caption*{VeriX \newline}
%     \end{subfigure}
%     \hfill
%     \begin{subfigure}[t]{0.09\textwidth}
%         \centering
%         \includegraphics[width=\textwidth]{diagrams/qualitative_result_for_experiment/mnist/lime.png}
%         \caption*{LIME \newline}
%     \end{subfigure}
%     \hfill
%     \begin{subfigure}[t]{0.09\textwidth}
%         \centering
%         \includegraphics[width=\textwidth]{diagrams/qualitative_result_for_experiment/mnist/anchors.png}
%         \caption*{Anchors \newline}
%     \end{subfigure}
%     \hfill
%     \begin{subfigure}[t]{0.09\textwidth}
%         \centering
%         \includegraphics[width=\textwidth]{diagrams/qualitative_result_for_experiment/mnist/ig.png}
%         \caption*{IG \newline}
%         \label{fig:ig}
%     \end{subfigure}
    
%     \vspace{-0.5em}
%     \caption{Qualitative results comparing the baselines (Targeted explanation from 4 to 9)}
%     \label{fig:comparison_to_table1}
%     \vspace{-1em}
% \end{figure}


% Please add the following required packages to your document preamble:
% \usepackage{multirow}
\begin{table*}[!t]
\small
\caption{Comparison of XAI methods in terms of fidelity (higher is better), time in seconds, cardinality (absolute pixels), and robustness to perturbations (higher is better). LIME does not compute the anchor region for the input, making our perturbation-based robustness metric inapplicable. Hence, we denote its robustness score with `–'.}
\label{tab:comprehensive}
\vspace{-0.5em}
\centering

\begin{tabular}{llcccccccc}
    \toprule
    & & \multicolumn{4}{c}{MNIST} & \multicolumn{4}{c}{GTSRB} \\
    \cmidrule(r){3-6} \cmidrule(r){7-10}
    \textbf{Method} & \textbf{Reach} 
      & \textbf{Fidelity} & \textbf{Time (sec)} & \textbf{Cardinality} & \textbf{Robust.}
      & \textbf{Fidelity} & \textbf{Time (sec)} & \textbf{Cardinality} & \textbf{Robust.} \\
    \midrule
    \textbf{ViTaX} & Approx 
        & \textbf{0.64} & \textbf{13.75} & \textbf{121.46} & 0.90 
        & \textbf{0.71} & \textbf{47.23} & \textbf{30.57}  & 0.82 \\
        %          & Exact 
        % & - & - & - & 1.00 
        % & - & - & - & 1.00 \\
    VeriX & 
        & 0.18 & 699.72 & 472.15 & 0.94
        & 0.20 & 1536.34 & 764.97 & 0.99 \\
    Brute Force & 
        & 0.36 & 1457.04 & 145.16 & 0.35
        & 0.29 &  7034.34 & 147.66 & 0.52 \\
    % - - -& 
    %     & -- & -- & -- & --
    %     & -- & -- & -- & -- \\
    \midrule
    LIME & 
        & 0.18 & 18.32 & 307.48 & --
        & 0.13 & 26.45 & 384.61 & -- \\
    Anchors & 
        & 0.17 & 16.73 & 44.89 & 0.21
        & 0.14 & 33.55 & 302.30 & 0.73 \\
    % IG & 
    %     & 0.33 & 0.01 & 238.49 & -
    %     & 0.01 & 0.01 & 408.39 & - \\
    \bottomrule
\end{tabular}
\end{table*}


% ViTaX Pos. & Sens. & Approx          & -               & -                & 0.45         & -               & -               & 0.29          \\
%                    ViTaX Neg. &  &           & -               & -                & 0.25         & -               & -               & 0.29          \\
%                  ViTaX Rand.   &  &           & -               & -                & 0.35          & -               & -               & 0.30          \\


% \vspace{-0.5em}

% \begin{table}[!ht]
% \small
%   \caption{Table for comparison between baselines of other XAI method and formal methods in fidelity (higher is better), time in sec, and cardinality in absolute pixels.}
%   \label{tab:comprehensive}
%   \centering
%   \begin{tabular}{llllllll}
%     \toprule
%     \multicolumn{2}{c}{} &
%     \multicolumn{3}{c}{MNIST} &
%     \multicolumn{3}{c}{GTSRB} \\
%     \cmidrule(r){3-5}
%     \cmidrule(r){6-8}
%     Method & Reach & Fidelity & Time & Cardinality & Fidelity & Time & Cardinality \\
%     \midrule
%     ViTaX & Approx & \textbf{0.64 + 0.41} & 13.75 + 3.9  & 121.46 + 53.1 & \textbf{0.71 + 0.41} & 47.23 + 30.6 & 30.57 + 49.36 \\
%            & Relax50  & 0.63 + 0.41 & 9.56 +2.35 & 111.14 +47.9 & 0.70 + .42 & 35.32 + 24.5 & 30.51 +49.3\\
%            %& Random  & 0.34 & 15.99 & 158.64 & 0.28 & 88.92 & 142.92 \\
%            %& IG & 0.37 & 14.16 & 124.11 & 0.38 & 52.29 & 42.50 \\

%     VeriX & & 0.18 & 699.72 & 472.15 & 0.2003 & 1536.34 & 764.97 \\
%     LIME  & & 0.35 & 0.65 & 556.65 & 0.27 & 0.77 & 374.54 \\
%     Anchors & & 0.166 & 0.0238 & 44.89 & 0.135 & 0.0131 & 302.30 \\
%     IG & & 0.18 & 0.00618 & 238.489 & 0.43 & 0.0063 & 389.67 \\
%     \bottomrule
%   \end{tabular}
% \end{table}
